Dudeney's Dissection is Optimal

In 1907, Henry Ernest Dudeney posed a puzzle: ``cut any equilateral triangle \dots\ into as few pieces as possible that will fit together and form a perfect square'' (without overlap, via translation and rotation). Four weeks later, Dudeney demonstrated a beautiful four-piece solution, which today remains perhaps the most famous example of dissection. In this paper (over a century later), we finally solve Dudeney's puzzle, by proving that the equilateral triangle and square have no common dissection with three or fewer polygonal pieces. We reduce the problem to the analysis of discrete graph structures representing the correspondence between the edges and the vertices of the pieces forming each polygon.

==> memo-C.tex <==
         %%%%%%%%%%%%           
        \textbf{\boldmath Case C-1:} 
        If $\VD$ contains a tadpole graph $L$, then the degree-2 corner vertex of $S$ (along with one of the degree-1 corner vertices) is included in $L$, and the tree $Y$ is well-behaved.
        Therefore, in this case, a contradiction can be derived using the same argument as in Case B.
        Therefore, we consider the case where $\VD$ consists of a well-behaved path $W$ and a tree $Y$ with a degree-4 vertex.
        Here, based on the presence or absence of a U-shape, we classify the cases as follows.
        \begin{itemize}
            \item \textbf{Case C-1-1:} $\{G^T_1\} \times \{G^S_9\}, \{G^T_3, G^T_4\} \times \{G^S_{19}, G^S_{26}, G^S_{28}\}$
            \item \textbf{Case C-1-1:} $\{G^T_1\} \times \{G^S_{10}\}, \{G^T_3, G^T_4\} \times \{G^S_{20}, G^S_{27}\}$
        \end{itemize}

        \textbf{\boldmath Case C-1-1: Case where a U-shape is present:}
        If both endpoints of $W$ are the endpoints of the U-shape, the conditions of Lemma~\ref{lem:U-shape} hold, leading to a contradiction, just as in Case A.
        Therefore, one endpoint of $W$ must be an endpoint of the U-shape, while the other must be a different corner vertex that is not part of the U-shape.

%%%%%%%%%%%%   
        In this case, there exists a well-behaved path $P$ connecting vertices of $S$ by Lemma~\ref{lem:struct_BandC}.
        As shown in Figure~\ref{fig:CaseC}, $N^{S}_{\mathit{dit}}(\VD)$ consists of points on either T-cut edges or edges of $S$, and the number of points on the edges of $S$ is at most two.
        Therefore, we give a case distinction depending on how many points on an edge of $S$ are included in $P$ and show that both cases are infeasible.
    
        \textbf{\boldmath Case C-1: $W$ includes two points $t$ and $t^{\prime}$ on edges of $S$:}
            This would be happen in $\{G^T_3,G^T_4\} \times \{G^S_{6}, G^S_{19}, G^S_{20}\}$, $\{G^T_1\} \times \{G^S_{3}, G^S_{9}, G^S_{10}\}$.
            In this case, we have two possibilities: either the two endpoints of $P$ are at the endpoints of an edge of $S$, or they are not. 
            Based on this, we proceed with a case distinction.
            
        \textbf{\boldmath Case C-1-1: both endpoints of $W$ are at the endpoints of an edge of $S$:}
            Here, there are two adjacent monochromatic edges (Figure~\ref{fig:CaseC-1-1}), which leads to a contradiction with Lemma~\ref{lem:adjacent}.

            \begin{figure}[htbp]\centering
                \includegraphics[width=\textwidth]{fig/CaseC-1-1.pdf}
                \caption{The case where both endpoints of $W$ are at the endpoints of an edge of $S$.}
                \label{fig:CaseC-1-1}
            \end{figure}
            
        \textbf{\boldmath Case C-1-2: the endpoints of $P$ are diagonal vertices of $S$:}
            Except for the cases of $G^S_{10}$ or $G^S_{20}$, there are two monochromatic edges that connect to $W$ with the same orientation (Figure~\ref{fig:CaseC-1-2}), which leads to a contradiction with Lemma~\ref{lem:adjacent}.

            \begin{figure}[htbp]\centering
                \includegraphics[width=0.5\textwidth]{fig/CaseC-1-2.pdf}
                \caption{the case where the endpoints of $W$ are not both at the endpoints of an edge of $S$.}
                \label{fig:CaseC-1-2}
            \end{figure}
            
            In the case of $G^S_{10}$ or $G^S_{20}$, there are only two monochromatic edges entering $W$ with different orientations, as shown on the left in Figure~\ref{fig:G_20orG_10}. 
            Since $P$ passes through both $t$ and $t^{\prime}$, the only possible structure is as shown on the right in Figure~\ref{fig:G_20orG_10}. 
            Applying Lemma~\ref{lem:alternate} to this configuration leads to the equation $4\sigma = 3\tau$, which is a contradiction.

            \begin{figure}[htbp]\centering
                \includegraphics[width=\textwidth]{fig/G_20orG_10.pdf}
                \caption{Possible configurations for $G^S_{10}$ or $G^S_{20}$.}
                \label{fig:G_20orG_10}
            \end{figure}
        
        \textbf{\boldmath Case C-2: $P$ includes one point $t$ on an edge of $S$:}
            In this case, it suffices to consider the scenario where the endpoints of $P$ are adjacent, and $t$ is included on the opposite side. 
            This is because if $t$ shares an edge of $S$ with either endpoint of $P$, there would either be an odd number of monochromatic edges or two adjacent ones, leading to contradictions as before.
            The case that the endpoints of $P$ are adjacent, and $t$ is included on the opposite side occurs only in $\{G^T_1\} \times \{G^S_{3}, G^S_{9}\}$ and $\{G^T_3, G^T_4\} \times \{G^S_{6}, G^S_{19}, G^S_{28}\}$. 
            Here, the only two possible structures are shown in Figure~\ref{fig:CaseC-2}. 
            The left configuration is infeasible because it leads to the equation $3\sigma = 2\tau$ by Lemma~\ref{lem:alternate}. 
            The right configuration implies that all vertices of $S$ not in $P$ and the reminder divide-in-two vertices are in the same connected component $Y$ which include the vertices of $T$.
            It means that $Y$ should be a tree with $5$ leaves and two points of degree $3$, which contain no cycle.
            The remaining two edges of $T$ must form a path in $\ED$, but since they are adjacent and the shared vertex in $Y$, this contradicts Lemma~\ref{lem:adjacent}.

            \begin{figure}[htbp]\centering
                \includegraphics[width=\textwidth]{fig/CaseC-2.pdf}
                \caption{Possible configurations in Case C-2.}
                \label{fig:CaseC-2}
            \end{figure}
        
        \textbf{\boldmath Case C-3: $P$ includes no points on edges of $S$:}
            In this case, we have two possibilities: either $W$ includes a point on T-cut edges, or they are not. 
            Based on this, we proceed with a case distinction.
        
        \textbf{\boldmath Case C-3-1: $P$ includes a point on T-cut edges:}    
            This occurs only in the case of $G^S_{16}$. 
            Here, the only two possible structures are shown in Figure~\ref{fig:CaseC-2}. 
            The left configuration is infeasible because it leads to the equation $3\sigma = 2\tau$ by Lemma~\ref{lem:alternate}. 
            The right configuration implies the remaining two edges of $T$ included in the along sequence of $W$ are adjacent and must form a path in $\ED$, contradicting Lemma~\ref{lem:adjacent}.

            \begin{figure}[htbp]\centering
                \includegraphics[width=\textwidth]{fig/CaseC-3.pdf}
                \caption{Possible configurations when $P$ includes a point on T-cut edges in Case C-3.}
                \label{fig:CaseC-3}
            \end{figure}
                
        \textbf{\boldmath Case C-3-2: $W$ includes no point on T-cut edges:}
            Let $p$ and $p^{\prime}$ be the pair of the endpoints of $P$.
            Let $e_1$ and $e_2$ be the edges that incident to $p$ clockwise and counterclockwise, respectively, and similarly define $e^{\prime}_1$ and $e^{\prime}_2$ for $p^{\prime}$.
            Here, either $e_1$ and $e^{\prime}_2$ or $e_2$ and $e^{\prime}_1$ serve as the endpoints of a path in $\ED$.
            By Observation, the lengths at the endpoints of the path are equal. 
            The cut edges on the boundary of $S$ are strictly shorter than $\sigma$. 
            Therefore, it is sufficient to consider only cases where the non-cutting edges incident to the endpoints of $P$ have the same orientation.
            Moreover, the pair that does not serve as the endpoints of a path in $\ED$ has a combined length of $\tau$ because the opposite endpoints of each path in $\ED$ form a bisected edge of $T$. 
            Therefore, these edges cannot form a single edge of $S$.
            From the above considerations, it is sufficient to consider only the case in ${G^S_{10}, G^S_{20}, G^S_{27}}$ (left of Figure~\ref{fig:CaseC-3-2}) where the diagonal vertices of $S$ are the endpoints of $P$, and the pairs of adjacent non-cutting edges form paths in $\ED$ (middle of Figure~\ref{fig:CaseC-3-2}).        
            In this case, consider a connected component $C$ which includes the bisected vertex of $S$. 
            The component $C$ must contain a cycle and the remaining vertex, because the non-cutting edges must be connected, and by Lemma~\ref{lem:VG-component}. 
            Therefore, $C$ should be a tadpole graph, obtained by joining a cycle graph to a path graph with a bridge of degree 3 (right of  Figure~\ref{fig:CaseC-3-2}).
            Thus, three vertices of $T$ are connected by a tree $Y$, and $Y$ is well-behaved because it does not contain the bisected vertex of $S$. 
            Since $Y$ is well-behaved, this reduces to Case B.
            \begin{figure}[htbp]\centering
                \includegraphics[width=\textwidth]{fig/CaseC-3-2.pdf}
                \caption{Possible configurations when $P$ includes no point on a flat node in Case C-3.}
                \label{fig:CaseC-3-2}
            \end{figure}
    \end{proof}
